Commonsense Video Question Answering through Video-Grounded Entailment Tree Reasoning

This paper proposes the first video-grounded entailment tree reasoning method for commonsense video question answering (VQA). Despite the remarkable progress of large visual-language models (VLMs), there are growing concerns that they learn spurious correlations between videos and likely answers, reinforced by their black-box nature and remaining benchmarking biases. Our method explicitly grounds VQA tasks to video fragments in four steps: entailment tree construction, video-language entailment verification, tree reasoning, and dynamic tree expansion. A vital benefit of the method is its generalizability to current video and image-based VLMs across reasoning types. To support fair evaluation, we devise a de-biasing procedure based on large-language models that rewrites VQA benchmark answer sets to enforce model reasoning. Systematic experiments on existing and de-biased benchmarks highlight the impact of our method components across benchmarks, VLMs, and reasoning types.

==> tables/benchmark.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cccccc|cccccc}
\hline
\multicolumn{2}{c|}{} &
  \multicolumn{6}{c|}{NExT-QA} &
  \multicolumn{6}{c}{IntentQA} \\ \cline{3-14} 
\multicolumn{2}{c|}{\multirow{-2}{*}{Model}} &
  Temp &
  Caus &
  \multicolumn{1}{c|}{Avg} &
  Temp* &
  Caus* &
  Avg* &
  Temp &
  Caus &
  \multicolumn{1}{c|}{Avg} &
  Temp* &
  Caus* &
  Avg* \\ \hline
\multicolumn{1}{c|}{} &
  BLIP-2 &
  38.3 &
  36.1 &
  \multicolumn{1}{c|}{37.2} &
  33.9 &
  30.1 &
  33.5 &
  43.8 &
  48.6 &
  \multicolumn{1}{c|}{46.2} &
  34.0 &
  42.4 &
  38.2 \\
\multicolumn{1}{c|}{} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}45.3 &
  \cellcolor[HTML]{E2E1E1}41.8 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}43.6} &
  \cellcolor[HTML]{E2E1E1}41.4 &
  \cellcolor[HTML]{E2E1E1}38.2 &
  \cellcolor[HTML]{E2E1E1}39.8 &
  \cellcolor[HTML]{E2E1E1}48.9 &
  \cellcolor[HTML]{E2E1E1}52.5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}50.7} &
  \cellcolor[HTML]{E2E1E1}41.3 &
  \cellcolor[HTML]{E2E1E1}49.7 &
  \cellcolor[HTML]{E2E1E1}45.5 \\ \cline{2-14} 
\multicolumn{1}{c|}{} &
  LLaVA-1.5 &
  37.8 &
  40.7 &
  \multicolumn{1}{c|}{39.3} &
  35.4 &
  34.1 &
  34.8 &
  45.8 &
  50.0 &
  \multicolumn{1}{c|}{47.9} &
  38.9 &
  46.5 &
  42.7 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Image-based\\ VLMs\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}45.6 &
  \cellcolor[HTML]{E2E1E1}47.9 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}46.8} &
  \cellcolor[HTML]{E2E1E1}44.3 &
  \cellcolor[HTML]{E2E1E1}45.5 &
  \cellcolor[HTML]{E2E1E1}44.9 &
  \cellcolor[HTML]{E2E1E1}48.4 &
  \cellcolor[HTML]{E2E1E1}54.7 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}51.6} &
  \cellcolor[HTML]{E2E1E1}45.2 &
  \cellcolor[HTML]{E2E1E1}51.9 &
  \cellcolor[HTML]{E2E1E1}48.6 \\ \hline
\multicolumn{1}{c|}{} &
  VideoChat2 &
  56.9 &
  62.1 &
  \multicolumn{1}{c|}{59.5} &
  46.0 &
  44.8 &
  45.4 &
  60.4 &
  63.2 &
  \multicolumn{1}{c|}{61.8} &
  51.3 &
  53.9 &
  52.6 \\
\multicolumn{1}{c|}{} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}57.8 &
  \cellcolor[HTML]{E2E1E1}61.6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}59.7} &
  \cellcolor[HTML]{E2E1E1}49.7 &
  \cellcolor[HTML]{E2E1E1}48.2 &
  \cellcolor[HTML]{E2E1E1}49.0 &
  \cellcolor[HTML]{E2E1E1}62.3 &
  \cellcolor[HTML]{E2E1E1}63.8 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}63.1} &
  \cellcolor[HTML]{E2E1E1}55.1 &
  \cellcolor[HTML]{E2E1E1}56.3 &
  \cellcolor[HTML]{E2E1E1}55.7 \\ \cline{2-14} 
\multicolumn{1}{c|}{} &
  VideoLLaVA &
  56.0 &
  60.4 &
  \multicolumn{1}{c|}{58.2} &
  48.8 &
  53.4 &
  51.1 &
  53.9 &
  60.7 &
  \multicolumn{1}{c|}{57.3} &
  48.4 &
  52.6 &
  50.5 \\
\multicolumn{1}{c|}{} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}58.3 &
  \cellcolor[HTML]{E2E1E1}62.7 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}60.5} &
  \cellcolor[HTML]{E2E1E1}53.1 &
  \cellcolor[HTML]{E2E1E1}57.6 &
  \cellcolor[HTML]{E2E1E1}55.4 &
  \cellcolor[HTML]{E2E1E1}57.6 &
  \cellcolor[HTML]{E2E1E1}61.8 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}59.7} &
  \cellcolor[HTML]{E2E1E1}53.8 &
  \cellcolor[HTML]{E2E1E1}55.5 &
  \cellcolor[HTML]{E2E1E1}54.7 \\ \cline{2-14} 
\multicolumn{1}{c|}{} &
  VideoLLAMA &
  55.4 &
  60.2 &
  \multicolumn{1}{c|}{57.8} &
  40.7 &
  42.3 &
  41.4 &
  55.1 &
  56.7 &
  \multicolumn{1}{c|}{55.9} &
  47.7 &
  44.9 &
  46.3 \\
\multicolumn{1}{c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Video-based\\ VLMs\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}58.1 &
  \cellcolor[HTML]{E2E1E1}60.4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}59.3} &
  \cellcolor[HTML]{E2E1E1}46.0 &
  \cellcolor[HTML]{E2E1E1}47.9 &
  \cellcolor[HTML]{E2E1E1}47.0 &
  \cellcolor[HTML]{E2E1E1}54.5 &
  \cellcolor[HTML]{E2E1E1}58.9 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}56.7} &
  \cellcolor[HTML]{E2E1E1}50.8 &
  \cellcolor[HTML]{E2E1E1}49.1 &
  \cellcolor[HTML]{E2E1E1}50.0 \\ \hline
\multicolumn{1}{c|}{} &
  VideoTree &
  67.0 &
  75.2 &
  \multicolumn{1}{c|}{71.1} &
  60.2 &
  66.4 &
  63.3 &
  61.9 &
  66.1 &
  \multicolumn{1}{c|}{64.0} &
  56.7 &
  60.1 &
  58.4 \\
\multicolumn{1}{c|}{} &
  VideoAgent &
  64.5 &
  72.7 &
  \multicolumn{1}{c|}{68.6} &
  58.2 &
  66.6 &
  62.9 &
  64.1 &
  66.5 &
  \multicolumn{1}{c|}{65.3} &
  60.4 &
  61.0 &
  60.7 \\
\multicolumn{1}{c|}{} &
  LLoVi &
  61.0 &
  69.5 &
  \multicolumn{1}{c|}{65.3} &
  53.1 &
  60.8 &
  57.0 &
  65.5 &
  68.7 &
  \multicolumn{1}{c|}{67.1} &
  58.6 &
  61.8 &
  60.2 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Video QA\\ Approaches\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}Ours &
  \cellcolor[HTML]{E2E1E1}64.8 &
  \cellcolor[HTML]{E2E1E1}71.7 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}68.3} &
  \cellcolor[HTML]{E2E1E1}\textbf{60.8} &
  \cellcolor[HTML]{E2E1E1}65.9 &
  \cellcolor[HTML]{E2E1E1}\textbf{63.4} &
  \cellcolor[HTML]{E2E1E1}\textbf{66.1} &
  \cellcolor[HTML]{E2E1E1}66.4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2E1E1}66.3} &
  \cellcolor[HTML]{E2E1E1}\textbf{61.0} &
  \cellcolor[HTML]{E2E1E1}\textbf{62.6} &
  \cellcolor[HTML]{E2E1E1}\textbf{61.6} \\ \hline
\end{tabular}%
}
\caption{Results on NExT-QA and IntentQA, experiments are conducted under both original and rewritten test sets. * indicates the rewritten QA set. \cs{On what model is ours based in the last row?}}
\label{tab:benchmark}
\end{table*}

==> tables/supp_breakdown_gnd.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{cc|cc}
\hline
\multicolumn{2}{c|}{Components}              & \multicolumn{2}{c}{Acc} \\ \hline
\begin{tabular}[c]{@{}c@{}}Fact-condition \\ captioning\end{tabular} & \begin{tabular}[c]{@{}c@{}}Structure-based \\ retrieval\end{tabular} & Original & Rewritten \\ \hline
\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & 56.2       & 49.6       \\
$\checkmark$                  &                       & 59.5       & 53.3       \\
                     & $\checkmark$                   & 58.4       & 52.7       \\
$\checkmark$                  & $\checkmark$                   & 60.5       & 55.4       \\ \hline
\end{tabular}%
}
\caption{Ablation study of our grounding part.}
\label{tab:supp_break_ground}
\end{table}

==> tables/supp_combination.tex <==
\begin{table}[t!]
\centering
\vspace{-3pt}
\begin{minipage}[t]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc|cccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{General VLM} & \multicolumn{4}{c}{VQA approaches}             \\ \cline{2-7} 
                        & VideoChat2      & VideoLlaVA     & VideoAgent & VideoTree & LLoVi & Ours          \\ \hline
Inf time(s)                & 7.5             & 6.2            & 51.0       & 34.6      & 40.3  & 38.2          \\ \hline
Avg acc                 & 49.0            & 50.8           & 61.6       & 60.9      & 58.6  & \textbf{62.6} \\ \hline
Reasoner &
  \begin{tabular}[c]{@{}c@{}}VideoChat2\\ (7B)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VideoLlaVA\\ (7B)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VideoLlaVA\\ (\textbf{7B})\end{tabular} \\ \hline
\end{tabular}%
}
\vspace{-10pt}
\caption{Efficiency comparison. The average inference time for each video is reported.}
\label{tab:supp_efficiency}
\end{minipage}
\begin{minipage}[t]{0.5\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|cc}
\hline
\multicolumn{2}{c|}{Components}              & \multicolumn{2}{c}{Acc} \\ \hline
\begin{tabular}[c]{@{}c@{}}Fact-\\ conditioned \\ captioning\end{tabular} & \begin{tabular}[c]{@{}c@{}}Structure-\\ based \\ retrieval\end{tabular} & Original & Rewritten \\ \hline
\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & 56.2       & 49.6       \\
yes                  &                       & 59.5       & 53.3       \\
                     & yes                   & 58.4       & 52.7       \\
yes                  & yes                   & 60.5       & 55.4       \\ \hline
\end{tabular}%
}
\vspace{-10pt}
\caption{Ablation study of main components in grounding part.}
\label{tab:supp_break_ground}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \begin{minipage}[t]{\linewidth}
    \centering
    \vspace{-1.3cm}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c}
    \hline
    Method          & Original set & De-basing set \\ \hline
    Human w/o video & 79.3         & 44.6          \\ \hline
    Human w/ video  & 96.4         & 93.9          \\ \hline
    \end{tabular}}
    \vspace{-10pt}
        \caption{Results of subjective human evaluation (NExT-QA).}
        \label{tab:supp_quality}
    \end{minipage}
    \vspace{1cm}
    \begin{minipage}[t]{\linewidth}
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{c|c|c|c}
    \hline
    Model       & NExT-QA & IntentQA & Avg                          \\ \hline
    VideoLlaMA3 & 61.4    & 59.7     & 60.6                         \\
    \rowcolor[HTML]{E2E1E1} 
    +Ours       & 63.2    & 60.9     & \cellcolor[HTML]{E2E1E1}62.1 \\ \hline
    \end{tabular}%
    }
    \vspace{-10pt}
        \caption{Results of VideoLlaMA3 w/ Ours.}
        \label{tab:supp_videollama3}
    \end{minipage}
    \end{minipage}
    \vspace{-1.3cm}
\end{table}

==> tables/supp_human.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{c|c|c}
\hline
Method          & Original set & De-basing set \\ \hline
Human w/o video & 79.3         & 44.6          \\ \hline
Human w/ video  & 96.4         & 93.9          \\ \hline
\end{tabular}%
}
\caption{Average results of the original set and de-basing set, which are answered by 3 people under (1) only observing the question-answers (2) watching both the video and question-answers}
\label{tab:supp_quality}
\end{table}

==> tables/supp_time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc|cccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{General VLM} & \multicolumn{4}{c}{VQA approaches}             \\ \cline{2-7} 
                        & VideoChat2      & VideoLlaVA     & VideoAgent & VideoTree & LLoVi & Ours          \\ \hline
Inf time(s)                & 7.5             & 6.2            & 51.0       & 34.6      & 40.3  & 38.2          \\ \hline
Avg acc                 & 49.0            & 50.8           & 61.6       & 60.9      & 58.6  & \textbf{62.6} \\ \hline
Reasoner &
  \begin{tabular}[c]{@{}c@{}}VideoChat2\\ (7B)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VideoLlaVA\\ (7B)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GPT-4\\ (1.8T)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VideoLlaVA\\ (\textbf{7B})\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Efficiency comparison. The average inference time for each video is reported. Acc is reported by the average accuracy on the de-biasing set of NExT-QA and Intent-QA.}
\label{tab:supp_efficiency}
\end{table}


%Efficiency comparison. The average inference time for each video in NExT-QA is reported.

==> tables/supp_videollama3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{c|c|c|c}
\hline
Model       & NExT-QA & IntentQA & Avg                          \\ \hline
VideoLlaMA3 & 61.4    & 59.7     & 60.6                         \\
\rowcolor[HTML]{E2E1E1} 
+Ours       & 63.2    & 60.9     & \cellcolor[HTML]{E2E1E1}62.1 \\ \hline
\end{tabular}%
}
\caption{Results of VideoLlaMA3 incorporating our framework.}
\label{tab:supp_videollama3}
\end{table}

==> tables/videomme.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|cccc}
\hline
\multicolumn{2}{c|}{} &
  \multicolumn{4}{c}{Accuracy} \\
\multicolumn{2}{c|}{\multirow{-2}{*}{Method}} &
  TR &
  SR &
  AR &
  OR \\ \hline
\multicolumn{1}{c|}{} &
  LLaVA &
  31.1 &
  33.6 &
  27.7 &
  29.8 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Image-based\\ VLMs\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}36.7 &
  \cellcolor[HTML]{E2E1E1}36.8 &
  \cellcolor[HTML]{E2E1E1}31.4 &
  \cellcolor[HTML]{E2E1E1}30.7 \\ \hline
\multicolumn{1}{c|}{} &
  VideoChat2 &
  50.3 &
  52.4 &
  49.5 &
  50.1 \\
\multicolumn{1}{c|}{} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}52.8 &
  \cellcolor[HTML]{E2E1E1}51.5 &
  \cellcolor[HTML]{E2E1E1}51.3 &
  \cellcolor[HTML]{E2E1E1}50.0 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  VideoLLaVA &
  47.6 &
  44.3 &
  46.2 &
  49.7 \\
\multicolumn{1}{c|}{} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}48.3 &
  \cellcolor[HTML]{E2E1E1}46.1 &
  \cellcolor[HTML]{E2E1E1}49.8 &
  \cellcolor[HTML]{E2E1E1}50.3 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  VideoLLaMA &
  44.8 &
  47.2 &
  44.7 &
  49.3 \\
\multicolumn{1}{c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Video-based\\ VLMs\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}+Ours &
  \cellcolor[HTML]{E2E1E1}47.4 &
  \cellcolor[HTML]{E2E1E1}47.8 &
  \cellcolor[HTML]{E2E1E1}48.6 &
  \cellcolor[HTML]{E2E1E1}49.1 \\ \hline
\multicolumn{1}{c|}{} &
  VideoTree &
  55.7 &
  54.3 &
  \textbf{54.2} &
  \textbf{52.6} \\
\multicolumn{1}{c|}{} &
  LLoVi &
  \multicolumn{1}{l}{52.2} &
  \multicolumn{1}{l}{\textbf{55.3}} &
  \multicolumn{1}{l}{51.8} &
  \multicolumn{1}{l}{51.0} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Video QA\\ Approches\end{tabular}}} &
  \cellcolor[HTML]{E2E1E1}Ours &
  \cellcolor[HTML]{E2E1E1}\textbf{55.9} &
  \cellcolor[HTML]{E2E1E1}53.8 &
  \cellcolor[HTML]{E2E1E1}54.0 &
  \cellcolor[HTML]{E2E1E1}50.8 \\ \hline
\end{tabular}%
}
\caption{Results of VideoMME short split, four QA types that focus on commonsense reasoning are selected. TR: temporal reasoning, SR: spatial reasoning, AR: action reasoning, OR: object reasoning}
\label{tab:videomme}
\end{table}
